From English-Centric to Effective Bilingual: LLMs with Custom Tokenizers for Underrepresented Languages

In this paper, we propose a model-agnostic cost-effective approach to developing bilingual base large language models (LLMs) to support English and any target language. The method includes vocabulary expansion, initialization of new embeddings, model training and evaluation. We performed our experiments with three languages, each using a non-Latin script - Ukrainian, Arabic, and Georgian. Our approach demonstrates improved language performance while reducing computational costs. It mitigates the disproportionate penalization of underrepresented languages, promoting fairness and minimizing adverse phenomena such as code-switching and broken grammar. Additionally, we introduce new metrics to evaluate language quality, revealing that vocabulary size significantly impacts the quality of generated text.

==> glossary.tex <==
\newglossaryentry{nlp}{
  name={NLP},
  first={Natural Language Processing (NLP)},
  description={Natural Language Processing (NLP) is a subfield of linguistics, computer science, and artificial intelligence concerned with the interactions between computers and human (natural) languages}
}
\newglossaryentry{llm}{
  name={LLM},
  first={Large Language Models (LLM)},
  description={You know what it is.},
  plural = {LLMs},
}
\newglossaryentry{nn}{
	name={NN},
	first={Neural Network (NN)},
	description={No idea what it is.},
	plural = {NNs}
}
\newacronym{lstm}{LSTM}{Long Short-Term Memory}
\newacronym{gru}{GRU}{Gated Recurrent Unit}
\newacronym{rnn}{RNN}{Recurrent Neural Networks}
\newacronym{cv}{CV}{Computer Vision}
\newacronym{RL}{RL}{Reinforced Learning}
\newacronym{DL}{DL}{Deep Learning}
\newacronym{gpt}{GPT}{Generative Pre-trained Transformer}
\newacronym{bert}{BERT}{Bidirectional Encoder Representations from Transformers}
\newacronym{eit}{EIT}{External Independent Testing}
\newacronym{mcq}{MCQ}{multiple choice questions}
\newacronym{oq}{OQ}{open questions}
\newacronym{xlu}{XLU}{cross-lingual
language understanding}
